Distributed Deterministic Exact Minimum Weight Cycle and Multi Source Shortest Paths in Near Linear Rounds in CONGEST model

We present new deterministic algorithms for computing distributed weighted minimum weight cycle (MWC) in undirected and directed graphs and distributed weighted all nodes shortest cycle (ANSC) in directed graphs. Our algorithms for these problems run in $\tilde{O}(n)$ rounds in the CONGEST model on graphs with arbitrary non-negative edge weights, matching the lower bound up to polylogarithmic factors. Before our work, no near linear rounds deterministic algorithms were known for these problems. The previous best bound for solving these problems deterministically requires an initial computation of all pairs shortest paths (APSP) on the given graph, followed by post-processing of $O(n)$ rounds, and in total takes $\tilde{O}(n^{4/3})$ rounds, using deterministic APSP~\cite{AR-SPAA20}. The main component of our new $\tilde{O}(n)$ rounds algorithms is a deterministic technique for constructing a sequence of successive blocker sets. These blocker sets are then treated as source nodes to compute $h$-hop shortest paths, which can then be used to compute candidate shortest cycles whose hop length lies in a particular range. The shortest cycles can then be obtained by selecting the cycle with the minimum weight from all these candidate cycles. Additionally using the above blocker set sequence technique, we also obtain $\tilde{O}(n)$ rounds deterministic algorithm for the multi-source shortest paths problem (MSSP) for both directed and undirected graphs, given that the size of the source set is at most $\sqrt{n}$. This new result for MSSP can be a step towards obtaining a $o(n^{4/3})$ rounds algorithm for deterministic APSP. We also believe that our new blocker set sequence technique may have potential applications for other distributed algorithms.

==> 2.tex <==
\subsection{Shortest Path Distances from $\sqrt{n}$ sources}

%first write the pseudocode
\begin{algorithm*}
% \scriptsize
\caption{$\sqrt{n}$ Multi-SSP Algorithm}
\begin{algorithmic}[1]
\Statex Input: $S$: set of sources, constant $\epsilon$: $1 > \epsilon > 0$
\State $i \leftarrow 0$; $Q_0 \leftarrow S$
\State Pick an integer $c$ such that $c > \log^{\epsilon} n$.
\While{$|Q_i| > c$} \label{algn12:while1}
\State $i \leftarrow i+1$; $h_i \leftarrow \sqrt{n}\cdot (\log n)^{1+\epsilon\cdot i}$
\State Compute $h_i$-CSSSP for set $Q_{i-1}$ using the algorithm in~\cite{AR19}. \label{algn12:computeCSSSP}
\State Compute a blocker set $Q_i$ of size $O(\sqrt{n}/\log^{\epsilon\cdot i} n)$ for the $h_i$-CSSSP computed in Step~\ref{computeCSSSP} using the algorithm in~\cite{AR20}.	\label{algn12:constructQ}
\EndWhile   \label{algn12:endWhile1}
\State $i' \leftarrow i$
\State \textbf{For each $\bm{c\in Q_{i'}}$ in sequence:} Compute shortest path distance values $\delta(c,x)$ at every node $x \in V$ using Bellman-Ford algorithm. \label{algn12:BF}
\While{$i > 0$} \label{algn12:startWhile2}
\State $i \leftarrow i-1$
\State \textbf{For each $\bm{c\in Q_{i+1}}$ in sequence:} Broadcast $ID(c)$ and the shortest path distance values $\delta_{h_{i+1}} (c',c)$ for each $c' \in Q_i$.	\label{algn12:broadcast}
\State \textbf{Local Step at node $\bm{x\in V}$:} Calculate the shortest path distance values for each $c'\in Q_i$ using Equation~\ref{} that uses the already computed shortest path distance values $\delta(c,x)$ for source nodes $c \in Q_{i+1}$, distance values $\delta_{h_{i+1}} (c',c)$ received in Step~\ref{algkSSP:broadcast} and $\delta_{h_{i+1}} (c',x)$ distance values computed at node $x$. \label{algn12:localCompute}
\EndWhile   \label{algn12:endWhile2}
\end{algorithmic}  \label{algn12}
\end{algorithm*} 

\subsubsection{Correctness of Algorithm~\ref{algn12}}

The following lemma is immediate from the blocker set algorithm in ~\cite{AR19}.

\begin{lemma} \label{lemma:algn12:while1}
At the end of every iteration of the while loop in 
Steps~\ref{algn12:while1}-\ref{algn12:endWhile1}, the following claim holds: 
$Q_i$ is a blocker set for the $h_i$-CSSSP collection computed in
Step~\ref{algn12:computeCSSSP} for set $Q_{i-1}$.
\end{lemma}

\begin{lemma}   \label{lemma:algn12:while2}
At the start of every iteration of the while loop in Steps~\ref{algn12:startWhile2}-\ref{algn12:endWhile2}, the following claim holds: every node $x \in V$ knows the shortest path distance value $\delta(s,x)$ from source nodes $s \in Q_i$.
\end{lemma}
\begin{proof}
Initially $i = i'$ and the claim holds for the source set $Q_{i'}$ since we compute shortest path distances from every node $s \in Q_{i'}$ using Bellman-Ford in Step~\ref{algn12:BF}.

Let $I$ be the largest $i$ for which this claim does not hold and it holds for all 
$i$ such that$i' \geq i > I$.
We now show that such an $I$ cannot exist.

Fix node $s \in Q_{I}$ and $t \in V$ such that the shortest path distance value 
$\delta (s,t)$ computed at $t$ is not correct.
Depending on the length of the shortest path from $s$ to $t$, we have the following
two cases:

\textit{Case $(i)$: If there is a shortest path from $s$ to $t$ that has less than or equal to $h_{I+1}$ hops,} 
then $t$ would have set $\delta (s,t) = \delta_{h_{I+1}} (s,t)$ in
Step~\ref{algn12:localCompute} using the $\delta_{h_{I+1}} (s,t)$ computed in 
Step~\ref{algn12:computeCSSSP}.

\textit{Case $(ii)$: All shortest paths from $s$ to $t$ have more than $h_{I+1}$ hops.}
Then using Lemma~\ref{lemma:algn12:while1}, 
there exists node $c \in Q_{I+1}$ such that 
$\delta(s,t) = \delta_{h_{i+1}} (s,c) + \delta (c,t)$.
Since the claim holds for $I$, $t$ knows the correct value of $\delta (c,t)$
and it would have received the value $\delta_{h_{i+1}} (s,c)$ in 
Step~\ref{algn12:broadcast} and thus would have correctly computed $\delta(s,t)$
in Step~\ref{algn12:localCompute} using these values.
This shows that such an $I$ cannot exist and hence the claim holds for all $i$.
\end{proof}

For the case when $i = 0$, $Q_0 = S$ and hence the following lemma is immediate
from Lemma~\ref{lemma:algn12:while2}.

\begin{lemma}
Algorithm~\ref{algn12} correctly computes the shortest path distance values from an arbitrary source set $S \subset V$ of size $\sqrt{n}$ to every other node in an $n$ node-graph $G = (V,E)$, undirected or directed, with arbitrary nonnegative edge-weights.
\end{lemma}

\subsubsection{Round Complexity of Algorithm~\ref{algn12}}

\begin{lemma}   \label{lemma:algn12:Qi}
The blocker set $Q_i$ constructed in Step~\ref{algn12:constructQ} of Algorithm~\ref{algn12} has size $O(\sqrt{n}/\log^{\epsilon\cdot i} n)$.
\end{lemma}
\begin{proof}
From Theorem~\ref{}, the size of the blocker set $Q_i$ is 
$O(n\log n/h_i) = O(\sqrt{n}/\log^{\epsilon\cdot i} n)$.
This establishes the lemma.
\end{proof}

\begin{lemma} \label{lemma:algn12:while1:iterations}
The while loop in Steps~\ref{algn12:while1}-\ref{algn12:endWhile1}
runs for at most $O(\frac{\log n}{\epsilon\log \log n})$ iterations in total.
\end{lemma}

\begin{proof}
The while loop terminates when size of set $Q_i$ goes below $c$.
From Lemma~\ref{lemma:algn12:Qi}, $|Q_i| = O(\sqrt{n}/\log^{\epsilon\cdot i} n)$.
Thus the largest value of $i$ such that $|Q_i| \leq c$ is
$\frac{1/2\cdot \log n - \log c}{\epsilon\cdot \log \log n}$
$ = O(\frac{\log n}{\epsilon\log \log n})$
\end{proof}

\begin{lemma}   \label{lemma:algn12:while1:rounds}
The while loop in Steps~\ref{algn12:while1}-\ref{algn12:endWhile1} takes $\tilde{O}(n)$ rounds in total.
\end{lemma}
\begin{proof}
Using Theorem~\ref{}, Step~\ref{algn12:computeCSSSP} takes 
$\tilde{O}(h_i\cdot |Q_{i-1}|) = \tilde{$
\end{proof}

\begin{lemma}
Algorithm~\ref{algn12} takes $\tilde{O}(n)$ rounds in total.
\end{lemma}

==> 3.tex <==
\subsection{Shortest Path Distances from $n^{2/3}$ sources}

%first write the pseudocode
\begin{algorithm*}
% \scriptsize
\caption{$n^{2/3}$ Multi-SSP Algorithm}
\begin{algorithmic}[1]
\Statex Input: $G = (V, E)$, $S$: set of sources, constant $\epsilon$: $1 > \epsilon > 0$
\State $i \leftarrow 0$; $Q_0 \leftarrow S$
\While{$|Q_i| > \sqrt{n}$}
\State $i \leftarrow i+1$; $h_i \leftarrow n^{1/3}\cdot (\log n)^{1+\epsilon\cdot i}$
\State Compute $h_i$-CSSSP for set $Q_{i-1}$ using the algorithm in~\cite{AR19}. \label{computeCSSSP}
\State Compute a blocker set $Q_i$ of size $O(n^{2/3}/\log^{\epsilon\cdot i} n)$ for the $h_i$-CSSSP computed in Step~\ref{computeCSSSP} using the algorithm in~\cite{AR20}.	\label{constructQ}
\EndWhile
\State Compute shortest path distance values from source nodes in $Q_{i'}$ to every other node in $G$ using Algorithm~\ref{algn12}. \label{computeInCSSSP}
\State Compute shortest path distance values from every node in $G$ to source nodes in $Q_{i'}$ by running Algorithm~\ref{algn12} on the reverse graph of $G$, $G^R$. (After this step, every node $x$ knows $\delta(x,c)$ values for each $c \in Q_{i'}$.) \label{computeInCSSSP}
\While{$i > 0$}
\State $i \leftarrow i-1$
\State Using Alg. 7 and 8 in~\cite{AR20}, propagate distance values $\delta(x,c)$ from nodes $x \in Q_i$ to nodes $c \in Q_{i+1}$. 
\State \textbf{For each $\bm{x\in Q_i}$ in sequence:} Compute \textit{extended} $h_{i+1}$-hop shortest paths starting from every $c \in Q_{i+1}$ using Bellman-Ford algorithm (Appendix~\ref{}) (After this step, every node $v\in V$ knows $\delta(x,v)$ values for each $x \in Q_i$.)
\EndWhile
\end{algorithmic}  \label{algAPSP}
\end{algorithm*} 

==> cycles.tex <==
\section{Finding Shortest Cycles}

%first write the pseudocode
\begin{algorithm*}
% \scriptsize
\caption{All Nodes Shortest Cycle Algorithm}
\begin{algorithmic}[1]
\Statex Input: $G = (V, E)$; number of hops $h = n^{1/6}$
\State Compute $h$-CSSSP for set $V$ using the algorithm in~\cite{AR19}. \label{computeCSSSP}
\State Compute a blocker set $Q$ of size $\tilde{O}(n/h)$ for the $h$-CSSSP computed in Step~\ref{computeCSSSP} using an algorithm in~\cite{AR20}.	\label{constructQ}
\State Compute shortest path distance values from source nodes in $Q$ to every other node in $G$ using Algorithm~\ref{algn12}. \label{algANSC:computeCSSSP}
\State Compute shortest path distance values from every node in $G$ to source nodes in $Q_{i'}$ by running Algorithm~\ref{algn12} on the reverse graph of $G$, $G^R$. (After this step, every node $x$ knows $\delta(x,c)$ values for each $c \in Q$.) \label{algANSC:computeInCSSSP}
\State Every node $x \in V$ sends distance value $\delta_h (s,x)$ for each neighbor node $s$ of $x$ computed in Step~\ref{computeCSSSP} to node $s$.    \label{algANSC:send-h-hop}
\State \textbf{For each $\bm{c\in Q}$ in sequence:} Every node $x \in V$ sends distance value $\delta (c,x)$ computed in Step~\ref{algANSC:computeCSSSP} to each of it's outgoing neighbors. \label{algANSC:send-c-x}
\State \textbf{Local Step at node $x \in V$:} Compute the weight of the shortest cycle that includes node $x$ using Equation~\ref{} that uses the distance values received in Steps~\ref{algANSC:send-h-hop} and \ref{algANSC:send-c-x}.
\end{algorithmic}  \label{algAPSP}
\end{algorithm*} 

==> multi-sssp.tex <==
\section{Multi Source Shortest Paths}

In this section we describe our near-linear rounds algorithm to compute shortest path 
distances from
an arbitrary set 
of $\sqrt{n}$ source nodes to every other node in a given graph $G = (V,E)$. 
%describe this here
%We first compute $(\sqrt{n}\log^{1+\epsilon} n)$-CSSSP for set $S$ using the algorithm
%in ~\cite{ARKP18}.
%We then compute a blocker set $Q$ of size $\frac{\sqrt{n}}{\log^{\epsilon} n}$ for
%this CSSSP collection
We compute a series of $h_i$-CSSSPs and their corresponding blocker sets $Q_i$,
until $|Q_{i^{'}}| = O(1)$ for some $i'$.
We then compute shortest path distances to every other node from the nodes in $Q_{i'}$
using Bellman-Ford.
We finally show how to obtain the shortest path distances from the original set of
$\sqrt{n}$ source nodes to every other node, by combining the 
computed shortest path distance
values from the nodes in $Q_{i'}$ along with the computed $h_i$-CSSSPs.
We describe this in detail in Section~\ref{}.

We then extend this to get a near-linear rounds algorithm for computing shortest path 
distances 
from a set of $n^{2/3}$ source nodes to every other node in the graph.
This is done by using an approach from ~\cite{AR20} and combining it with the above algorithm.
We then generalize this result for an arbitrary-sized set $S$ of source nodes.
This is described in Section~\ref{}.

\input{n1:2}

\input{n2:3}
